On Moving Object Segmentation from Monocular Video with Transformers

Moving object detection and segmentation from a single moving camera is a challenging task, requiring an understanding of recognition, motion and 3D geometry. Combining both recognition and reconstruction boils down to a fusion problem, where appearance and motion features need to be combined for classification and segmentation. In this paper, we present a novel fusion architecture for monocular motion segmentation - M3Former, which leverages the strong performance of transformers for segmentation and multi-modal fusion. As reconstructing motion from monocular video is ill-posed, we systematically analyze different 2D and 3D motion representations for this problem and their importance for segmentation performance. Finally, we analyze the effect of training data and show that diverse datasets are required to achieve SotA performance on Kitti and Davis.

==> problem.tex <==
Based on a pinhole camera model, projection and backprojection are defined as:
\begin{align}
\pi\left(\textbf{X} \right) &= 
\begin{bmatrix}
f_{x}\frac{X}{Z} + c_{x}, & f_{y}\frac{Y}{Z} + c_{y} \\
\end{bmatrix} \\
\pi^{-1}\left(\textbf{x},\; Z \right) &= 
\begin{bmatrix}
Z\frac{u-c_{x}}{f_{x}}, & Z\frac{v-c_{y}}{f_{y}}, & Z, & 1
\end{bmatrix}^{T}
\label{eq:projection}
\end{align}
with camera coordinates $ \textbf{x} = \left[ u,\; v,\; 1 \right] $, 3D coordinates $ \textbf{X} = \left[ X,\; Y,\; Z,\; 1 \right]^{T} $ and 
camera intrinsics $ \left[ f_{x},\; f_{y},\; c_{x},\; c_{y} \right] $. The camera motion is modelled using the rigid body motion $ \textbf{g}_{ij} \in SE_{3} $. Given two views $ i $ and $ j $, the relative coordinate transformation is defined as:
\begin{align}
\textbf{x}^{j} = \pi\left( \textbf{g}_{ij} \textbf{X}^{i} \right) &= \pi\left( \textbf{g}_{j}\textbf{g}^{-1}_{i} \pi^{-1}\left( \textbf{x}^{i},\; Z \right)  \right) \\
& = \Psi\left( \textbf{g}_{ij},\; \textbf{x}^{i},\; Z \right) ,\; \nonumber
\label{eq:view2view}
\end{align}
where $ \Psi $ is the reprojection operator that transforms a pixel coordinate from camera $ i $ into camera $ j $. Given an element of the Lie group $ \textbf{g} $, the logarithm map $ \xi = \log \textbf{g} \in se_{3} $ maps to the Lie algebra. Vice versa the exponential map is defined as $ \textbf{g} = e^{\xi} \in SE_{3} $.

==> tables/ablation_modality_neg_examples.tex <==
% Shared table for single-modality experiments
\begin{center}
	\begin{minipage}[c]{0.3\textwidth}
		\centering
		\resizebox{1.0\textwidth}{!}{%				
			\begin{tabular}{lccccc}
				\toprule
				&  & $ p_{neg} $ &  $ AP_{50} \uparrow $ & FP $ \downarrow $ & FN $ \downarrow $ \\
				\midrule
				\cellcolor{Dandelion} & & 0 & 15.55 & \textbf{14.42} & 107.8 \\
				\cellcolor{Dandelion} & \multirow{-2}{*}{\textbf{Kitti}} & 30 & \textbf{37.16} & 23.38 & \textbf{83.19} \\
				\midrule
				\cellcolor{BlueGreen} & & 0 & 19.846 & 897.90 & 263.85 \\
				\cellcolor{BlueGreen} & \multirow{-2}{*}{\textbf{Davis}} & 30 & \textbf{23.98} & \textbf{616.53} & \textbf{258.81} \\
				\bottomrule
			\end{tabular}
		}		
		\label{tab:neg}
		\captionof{table}{Ablation of neg. examples augmentation (FP and FN are not normalized). Experiments were run on Mix 1 with image and optical flow data.}
	\end{minipage}
	\begin{minipage}[c]{0.65\textwidth}
		\centering
		\setstackgap{L}{9pt}
		\begin{center}
		\resizebox{0.8\textwidth}{!}{%
			\begin{tabular}{lcccccccc}
				\toprule
				& & & \multicolumn{3}{c}{\textbf{Kitti}} & \multicolumn{3}{c}{\textbf{Davis}} \\
				Data & Modality & \Centerstack[c]{Fusion\\mechanism} & \cellcolor{Dandelion} $ AP_{50} \uparrow $ & \cellcolor{Dandelion} FP $ \downarrow $ & \cellcolor{Dandelion} FN $ \downarrow $ & \cellcolor{BlueGreen} $ AP_{50} \uparrow $ & \cellcolor{BlueGreen} FP $ \downarrow $ & \cellcolor{BlueGreen} FN $ \downarrow $ \\
				\midrule
				& & \cellcolor{light-gray} D & \cellcolor{light-gray} 37.16 & \cellcolor{light-gray} 0.12 & \cellcolor{light-gray} 0.41 & \cellcolor{light-gray} 23.98 & \cellcolor{light-gray} 0.39 & \cellcolor{light-gray} 0.16  \\
				& \multirow{-2}{*}{RGB + OF} & \cellcolor{lighter-gray} E+D & \cellcolor{lighter-gray} 39.65 & \cellcolor{lighter-gray} 0.15 & \cellcolor{lighter-gray} 0.40 & \cellcolor{lighter-gray} 35.88 & \cellcolor{lighter-gray} 0.29 & \cellcolor{lighter-gray} 0.15 \\
				& & D & 27.5 & 0.05 & 0.50 & 19.25 & 0.30 & 0.19 \\
				& \multirow{-2}{*}{RGB + SF} & E+D & 26.5 & 0.10 & 0.49 & 15.4 & 0.11 & 0.23 \\
				& & \cellcolor{light-gray} D & \cellcolor{light-gray} 27.6 & \cellcolor{light-gray} \textbf{0.05} & \cellcolor{light-gray} 0.50 & \cellcolor{light-gray} \textcolor{gray}{21.8} & \cellcolor{light-gray} \textcolor{gray}{0.38} & \cellcolor{light-gray} \textcolor{gray}{0.14} \\
				& \multirow{-2}{*}{RGB + SF*} & \cellcolor{lighter-gray} E+D & \cellcolor{lighter-gray} 37.8 & \cellcolor{lighter-gray} 0.33 & \cellcolor{lighter-gray} 0.38 & \cellcolor{lighter-gray} \textcolor{gray}{38.4} & \cellcolor{lighter-gray} \textcolor{gray}{0.13} & \cellcolor{lighter-gray} \textcolor{gray}{0.17} \\
				& & D & 27.6 & \textbf{0.05} & 0.50 & - & - & - \\
				& \multirow{-2}{*}{RGB + SF**} & E+D & 51.0 & 0.10 & 0.35 & - & - & - \\
				& & \cellcolor{light-gray} D & \cellcolor{light-gray} 29.51 & \cellcolor{light-gray} \underline{0.06} & \cellcolor{light-gray} 0.47 & \cellcolor{light-gray} 27.47 & \cellcolor{light-gray} 0.30 & \cellcolor{light-gray} 0.17 \\
				\multirow{-10}{*}{Mix 1} & \multirow{-2}{*}{RGB + Cost} & \cellcolor{lighter-gray} E+D & \cellcolor{lighter-gray} 47.9 & \cellcolor{lighter-gray} 0.22 & \cellcolor{lighter-gray} 0.35 & \cellcolor{lighter-gray} 33.27 & \cellcolor{lighter-gray} 0.49 & \cellcolor{lighter-gray} 0.14 \\
				\midrule
				& \multirow{2}{*}{RGB + OF} & D & \underline{70.82} & 0.32 & \underline{0.16} & 54.01 & 0.13 & \textbf{0.01} \\
				& & E+D & 60.88 & 0.29 & 0.24 & \underline{61.12} & 0.11 & 0.12 \\
				& & \cellcolor{light-gray} D & \cellcolor{light-gray} \textbf{72.07} & \cellcolor{light-gray} 0.31 & \cellcolor{light-gray} \textbf{0.16} & \cellcolor{light-gray} 58.76 & \cellcolor{light-gray} 0.11 & \cellcolor{light-gray} 0.13 \\
				& \multirow{-2}{*}{RGB + SF}  & \cellcolor{lighter-gray} E+D & \cellcolor{lighter-gray} 56.3 & \cellcolor{lighter-gray} 0.38 & \cellcolor{lighter-gray} 0.27 & \cellcolor{lighter-gray} 53.9 & \cellcolor{lighter-gray} \textbf{0.08} & \cellcolor{lighter-gray} 0.15 \\
				& & D & 68.46 & 0.26 & 0.21 & 58.40 & \underline{0.09} & 0.13 \\
				\multirow{-6}{*}{Mix 3} & \multirow{-2}{*}{RGB + Cost} & E+D & 65.12 & 0.22 & 0.23 & \textbf{64.10} & 0.11 & \underline{0.12} \\
				\bottomrule
		\end{tabular}
		}
		\end{center}
		\label{tab:tab5}
		\captionof{table}{Fusion of appearance with different modalities.\newline* denotes abs. scale depth ** denotes stereo depth}
	\end{minipage}
\end{center}

==> tables/all_single_modality.tex <==
% Shared table for single-modality experiments
\begin{center}
	\begin{minipage}[c]{0.4\textwidth}
		\centering
		\resizebox{1.0\textwidth}{!}{%
			\begin{tabular}{lccc}
				\cellcolor{lighter-gray} \fns{Modality} & \cellcolor{lighter-gray} \fns{$ AP $} & \cellcolor{lighter-gray} \fns{$ AP_{50} $} & \cellcolor{lighter-gray} \fns{$ AP_{75} $}  \\
				\midrule
				\fns{RGB} & \fns{56.53} & \fns{76.71} & \fns{57.5} \\
				\midrule
				\fns{Scene Flow$^{\dagger} $} & \fns{\textbf{75.19}} & \fns{\textbf{89.52}} & \fns{\textbf{77.03}} \\
				\fns{Optical Flow$^{\dagger} $} & \fns{\underline{72.24}} & \fns{\underline{87.43}} & \fns{\underline{74.52}} \\
				\fns{Scene Flow \cite{teed2021raft}} & \fns{55.39} & \fns{75.31} & \fns{56.26} \\
				\fns{Motion embedding \cite{neoral2021monocular}} & \fns{53.30} & \fns{75.20} & \fns{54.9} \\
				\fns{Optical Flow \cite{teed2020raft}} & \fns{52.45} & \fns{72.75} & \fns{52.73} \\
				\bottomrule
			\end{tabular}
		}
		\label{tab:tab1}
		\captionof{table}{Comparison input data for motion segmentation on FlyingThings3D. $ ^{\dagger} $ denotes ground truth.}
	\end{minipage}
	\begin{minipage}[c]{0.55\textwidth}
		\centering
		\setstackgap{L}{9pt}
		\resizebox{1.0\textwidth}{!}{%
			\begin{tabular}{lccccccc}
				\toprule
				& \multicolumn{3}{c}{\textbf{Kitti}} & \multicolumn{3}{c}{\textbf{Davis}} \\
				Modality & \cellcolor{Dandelion} $ AP_{50} \uparrow $ & \cellcolor{Dandelion} FP $ \downarrow $ & \cellcolor{Dandelion} FN $ \downarrow $ & \cellcolor{BlueGreen} $ AP_{50} \uparrow $ & \cellcolor{BlueGreen} FP $ \downarrow $ & \cellcolor{BlueGreen} FN $ \downarrow $ \\
				\midrule
				RGB (Coco) & \textbf{58.2} & 1.34 & \textbf{0.17} & \textbf{50.51} & 0.92 & \textbf{0.07} \\
				Optical Flow \cite{teed2020raft} & 25.1 & 0.99 & 0.43 & 30.2 & 0.63 & 0.13 \\
				\Centerstack{Scene Flow \cite{teed2021raft} \\ rel. scale} & 29.6 & 0.54 & 0.42 & 11.0 & \textbf{0.24} & 0.22 \\
				\Centerstack{Scene Flow \cite{teed2021raft} \\ abs. scale} & 36.8 & \underline{0.50} & 0.40  & \textcolor{gray}{39.84} & \textcolor{gray}{0.41} & \textcolor{gray}{0.14} \\
				\Centerstack{Scene Flow \cite{teed2021raft} \\ stereo} & \underline{44.4} & \textbf{0.10} & \underline{0.40} &  - & - & - \\
				\Centerstack{Motion \\ embedding \cite{neoral2021monocular}} & 28.9 & 0.59 & 0.43 & \underline{33.9} & \underline{0.57} & \underline{0.13} \\
				\bottomrule
			\end{tabular}
		}
		\label{tab:tab2}
		\captionof{table}{Zero-shot performance single-modality models on KITTI/Davis.	
			Grey results are for selected clips, where SfM reconstruction is possible.}
	\end{minipage}
\end{center}


